Towards Zero-resource Cross-lingual Entity Linking

Cross-lingual entity linking (XEL) grounds named entities in a source language to an English Knowledge Base (KB), such as Wikipedia. XEL is challenging for most languages because of limited availability of requisite resources. However, much previous work on XEL has been on simulated settings that actually use significant resources (e.g. source language Wikipedia, bilingual entity maps, multilingual embeddings) that are unavailable in truly low-resource languages. In this work, we first examine the effect of these resource assumptions and quantify how much the availability of these resource affects overall quality of existing XEL systems. Next, we propose three improvements to both entity candidate generation and disambiguation that make better use of the limited data we do have in resource-scarce scenarios. With experiments on four extremely low-resource languages, we show that our model results in gains of 6-23% in end-to-end linking accuracy.

==> 3z.old_method.tex <==
\section{Baseline Model}\label{baseline}
In this section, we describe existing methods for the candidate generation and the disambiguation, and use these to formulate our baseline XEL system, which is heavily inspired by existing works for (X)EL \cite{ling2015design, pan2017cross}. 
% Notably, these techniques rely heavily on the resources like $\mathbbm{W}_{\textrm{src}}$ which are not likely to be available in truly low-resource settings,
Notably, while these techniques are applicable to low-resource settings, they do not fully exploit the language-invariant resource and combine them in an efficient way, 
% while neglects the potential of language-invariant resource $\mathbbm{W}_{\textrm{eng}}$. 
% Firstly; secondly, the feature set of this baseline model does not fully exploit the language-invariant resource $\mathbbm{W}_{eng}$, resulting in its ignorance of important disambiguation clues; finally, 
an issue we attempt to rectify in our proposed method of Section \ref{model}.
% \gn{I think this section has lost the focus on resource constraints. If these baseline systems exist, why don't they solve all our problems in low resource settings? What should the readers be paying attention to when they read this section, as shortcomings of the existing methods? I think maybe one sentence here would be good. Also in 3.2 and 3.3, why are these not sufficient?}

% 
% we introduce previous methods that require access to $\mathbbm{W}_{\textrm{eng}}$, $\mathbbm{W}_{\textrm{src}}$ and $\mathbbm{M}$.
% We gradually make more strict resource availability constraints and incorporate resource-lighted components until reach the minimal resource requirement we are aware of in previous work: ($\mathbbm{RC}_1$, $\mathbbm{RC}_3$).
% We further improve the baseline model to accommodate extremely limited resource setting. The details of our proposed methods are introduced in Section \ref{model}.  

\subsection{Candidate Generation}\label{sec:candidate_generation}
\textsc{WikiMention}: With access to all the resources we list above, there is a straightforward approach to the candidate generation process, used by most state-of-the-art work in XEL~\cite{sil2018neural,upadhyay2018joint}.
Specifically, a monolingual mention-entity map can be extracted from $\mathbbm{W}_{\textrm{src}}$ by finding all cross-article links in $\mathbbm{W}_{\textrm{src}}$, and using the anchor text as $m$ and the linked entity as $e^\textrm{src}$. These entities are then redirected to English Wikipedia with $\mathbbm{M}$ to obtain $e$. For instance, if mention ``Neezerlaandi'' is linked to entity ``Neezerlaandi'' 
% \gn{it's not clear which one is the entity and which is the mention here. Maybe do the convention of marking entities using \texttt{typewriter font} (throughout the paper, and explaining it the first time you use this convention).} 
in some Oromo Wikipedia pages, the corresponding English Wikipedia entity ``Netherlands'' will be acquired through $\mathbbm{M}$ and used as a candidate entity for the mention. The prior score $p(e_{i,j}|m_i)$ provided by this model shows the \emph{probability} of linking to $e_{i,j}$ when mentioning $m_{i}$. % We use the existing implementation by~\citet{upadhyay2018joint}.\footnote{https://github.com/shyamupa/wiki\_candgen}
% To expand coverage, for a mention $m_i$ in the document, we also consider the candidate entities of any other mention $m_k$ if $m_i$ is the substring of $m_k$. \gn{Connecting this to the example above would be helpful}. 

Because of its heavy reliance on  $\mathbbm{W}_{\textrm{src}}$ and $\mathbbm{M}$, \textsc{WikiMention} does not generalize well to real low-resource settings where these resources are scarce. We discuss this in detail in Section~\ref{comparision}.

% \textsc{Translate}: To work in more realistic resource-limited settings, \citet{pan2017cross} propose a translation-based method that eliminates the necessity for $\mathbbm{W}_{\textrm{src}}$, which \textsc{WikiMention} is heavily reliant on. 
% In this method, mention $m$ in the source language is first translated to English with the help of bilingual entity map $\mathbbm{M}$.
% A list of candidate entities is then retrieved using the English mention-entity map extracted from $\mathbbm{W}_{\textrm{eng}}$. 
% % One side product of this candidate generation method is that we could obtain $f_l^1$ without accessing $\mathbbm{RC}_2$ too \sr{the features havent been introduced yet, can we move/remove this line?}. 
% %To our best knowledge, this is the method with the lowest resource dependency that performs full entity linking and disambiguation that we could find in the literature \gn{We need to make sure that it's clear why we don't consider Shruti's method to be ``prior work''}. 
% \smallskip

\textsc{Pivoting}: Recently,~\citet{rijhwani19aaai} propose a zero-shot transfer learning method for XEL candidate generation, which uses no resources in the source language. A character-level LSTM is trained to encode entities using a bilingual entity map between some high-resource language and English. If the chosen high-resource language is closely-related (same language family, shared orthography etc.) to the source language, the zero-shot transfer is successful in generating candidates for XEL. In this case, the prior $p(e_{i,j}|m_i)$ indicates similarity score. 
One disadvantage of this light resource-reliant \textsc{Pivoting} is its agnostics to the salience of an entity when referring a mention, which has proven informative in XEL~\cite{sil2018neural, upadhyay2018joint}. To make the best use of scarce but existent resource, we proposed a calibrated combination of \textsc{WikiMention} and \textsc{Pivoting} in Section \ref{sec:calibration}.

% The performance of a candidate generation method is measured by \emph{gold candidate recall}, the proportion of mentions whose candidate list contains the correct linked entity over all test mentions. Gold candidate recall is the upper bound on performance of an entity disambiguation system. 

Following previous work \cite{upadhyay2018joint, sil2018neural}, we consider \textsc{WikiMention} as the baseline candidate generation model. 

\subsection{Linear Featurization and Scoring}\label{sec:base_inference}

% \gn{I feel it's a bit strange to have ``Featurization and Model'', then ``Inference''. It seems like it'd be better to have ``Model and Inference'' then ``Featurization''. It'd actually probably be even better to have features first, but I can't think of any good way to describe the features before describing the model. Do you think we could restructure the sections a bit?}

Next, we move to the entity disambiguation step. Unfortunately for low-resource settings, many XEL disambiguation methods have extensive resource requirements such as $\mathbbm{M}$ and $\mathbbm{W}_{\textrm{src}}$ \cite{sil2018neural, upadhyay2018joint}. However, some previous work on XEL does limit its resource usage to $\mathbb{W}_{\text{eng}}$, which is available regardless of the language. Our baseline follows one such method by \citet{pan2017cross}.

%\sr{could we have a citation in the beginning of this section? until you get to the end, it sounds like we are proposing this model. we can say something like "inspired by Pan et al"}
%\sr{I meant that we kind of merge the last paragraph here since we are referring to the Pan et al paper there as well}
% \sr{also highlight what resources are needed to train the base model}\sz{The resource requirements are highlighted in 4.2}
Our baseline defines the score of associating a mention with an entity through two components: a \emph{local score} ($s_l$) that indicates the similarity between an entity and the local context in which it lies; and a \emph{global score} ($s_g$) that quantifies the similarity between an entity and other linked entities in the same document~\cite{ganea2016probabilistic, yamada2017learning, pan2017cross, ganea2017deep, le-titov-2018-improving}. On the log scale, the score of each entity is defined as:
\begin{equation}\label{burn:final}
    s(e_{i, j}|D)=s_g(e_{i, j}|D) + s_l(e_{i, j}|D)
\end{equation}

The local score is the linear combination of unary features $f_l^i(e_{i,j}) \in \mathbf{\Phi}(e_{i,j})$:
\begin{equation}\label{eq:base_l}
    s_l(e_{i,j}|D)={\Wv_l^T}\mathbf{\Phi}(e_{i,j})
\end{equation}
where $\textbf{W}_l \in \mathbbm{R}^{d_l \times 1}$ and $d_l$ is the number of unary features in the vector.

As seen in the top half of Table~\ref{tab:1}, a unary feature function takes one argument $e_{i,j}$ and returns a value that represents some property of this entity~\cite{globerson2016collective,pan2017cross}. Specifically, the grayed mention-entity prior $f_l^1(e_{i,j})$ is the main unary feature used by \citet{pan2017cross}, and we use this in our baseline.

%\sr{can you reference the table here and also bring it up to this page or the next page, since we're introducing the features here} 

On the other hand, the global score $s_g$ is an aggregation of entity pair scores $s_e$. Similarly, $s_e$ is measured by the linear combination of binary features $f_g^i(e_{i,j}, e_{k, w}) \in \mathbf{\Psi}(e_{i, j}, e_{k, w})$:
\begin{equation}\label{eq:base_e}
    s_e(e_{i,j}, e_{k, w})={\Wv_g^T}\mathbf{\Psi}(e_{i,j}, e_{k, w})
\end{equation}
% where $\textbf{W}_g \in \mathbbm{R}^{d_g \times 1}$ and $d_g$ is the number of binary features in the vector. 
Each binary feature function $f_g^i(e_{i,j}, e_{k, w})$ takes two entities as arguments, and returns a value that indicates the relatedness between the entities; as seen in the bottom half of Table ~\ref{tab:1}. Similarly to the unary case, the grayed co-occurrence feature $f_g^1(e_{i, j}, e_{k, w})$ is used in the baseline. We refer to these two grayed features as \textsc{Base}.

While these features have proven useful in higher-resource XEL, in lower-resource scenarios, we hypothesize that it is more important to design features that make the most of the language-invariant resource $\mathbbm{W}_{\textrm{eng}}$ to make up for the relative lack of other resources in the source language. We discuss more intelligent features in Section~\ref{feature}. 

% \st{To obtain $f_l^1(e_{i,j})$, we need to calculate $f_l^1(e_{i,j}^{\textrm{src}})$ in $\mathbbm{W}_{\textrm{src}}$, and use $\mathbbm{M}$ to map it to $e_{i,j}$. $f_g^1(e_{i, j}, e_{k, w})$ is collected from $\mathbbm{W}_{\textrm{eng}}$. These two features form the \textsc{Base} feature set. For simplicity, we omit the arguments of the feature functions described below.}


\subsection{Greedy Inference}\label{base_greedy}

Next, we must combine these scores to find an optimal entity assignment. Following \citet{ling2015design} and \citet{globerson2016collective}, we use the entity pair score to calculate the mention evidence $s_m(m_k, e_{i,j})$, indicating the relatedness between an entity and a mention; the mention evidence is selected in a greedy manner:
%\sr{I changed this quite a bit, could you check that it's correct?}:
\begin{equation}\label{eq:base_m}
    s_m(m_k, e_{i,j}) = \max_{e_{k,w}\in \Ev_{k}}(s_e(e_{i, j}, e_{k, w}))
\end{equation}
The global score is defined as the average of mention evidence across the document:
\begin{equation}\label{eq:base_g}
    s_g(e_{i,j}|D)=\frac{1}{|\Mv_{D}|}\sum_{k \neq i}s_m(m_k, e_{i,j})
\end{equation}
We refer to this inference model as \textsc{Greedy}. 

The greedy strategy often results in a sub-optimal assignment as the confidence of each candidate entity is not taken into consideration. To solve this problem, we propose to iteratively update belief of each candidate entity in Section \ref{sec:burn}.

We denote \textsc{WikiMention}+\textsc{Base}+\textsc{Greedy} as the end-to-end baseline system. 
% The features of the baseline model are shown in Table \ref{tab:1} (local features) and Table \ref{tab:2} (global features), highlighted with a gray background. This feature set is referred to as \textsc{Base}. A detailed description of the features is in Section \ref{feature}. 


%$f_l^1(e_{i,j})$: the mention-entity prior probability, and $f_g^1(e_{i, j}, e_{k, m})$: the co-occurrence probability of entity $e_{i,j}$ and entity $e_{k, m}$ of mention $m_k$. We show detailed formulations of these features in Table \ref{tab:1} and Table \ref{tab:2}. For simplicity, we omit arguments of each feature function in the following paragraphs. 

\input{unary_table.tex}
%\input{binary_table.tex}

\section{Proposed Model} \label{model}
%\sr{change this sentence to reflect something like "as shown in the previous section, existing entity linking methods require X resources for candidate generation and inference (CITE)} 
% As shown in the previous section, existing entity linking methods require at least English Wikipedia ($\mathbbm{W}_{\textrm{eng}}$) and a bilingual entity map ($\mathbbm{M}$) for candidate generation and inference.
% However, even the availability of $\mathbbm{M}$ is scarce for most living languages, making it almost impossible to directly apply these systems to languages with extremely limited resources. 
%\sr{the following sentence has been said in the intro, so we probably don't need to restate} In addition, even in languages where source Wikipedia ($\mathbbm{W}_{\textrm{src}}$) is available, often it can be small to the extent where it is not possible to rely on this resource heavily for either candidate generation or feature extraction.\sz{claims here are overlap}
% In this section, we introduce an XEL inference system that requires only the language-invariant resource $\mathbbm{W}_{\textrm{eng}}$, \emph{a first step towards real zero-resource XEL}. 
In this section, we first introduce a method for calibrated combination of two existing candidate generation models.
Then introduce our XEL disambiguation model that makes best use of the resources that will be available in extremely low-resource settings. % As it only requires the language-invariant resource $\mathbbm{W}_{\textrm{eng}}$, it is ready to be plugged into any XEL systems without bringing new resource requirements. It is \emph{a first step towards real zero-resource XEL}. 
Because the inference model is model is entirely language-agnostic, it is ready to be plugged into any XEL systems without re-training -- \emph{a first step towards true zero-resource XEL}. 

\subsection{Calibrated Candidate List Combination}\label{sec:calibration}
As the gold candidate recall decides the upper bound of an (X)EL system, candidate lists with close to 100\% recall are ideal. However, this is hard to achieve for most low resource languages where existing candidate generation models could only provide candidate lists with low recall (less than 60\%, as we show in experiments). What is worse, the combination of candidate lists retrieved by different models is non-trivial as the scores are not comparable among models. For example, the score of \textsc{WikiMention} has a probabilistic interpretation while the score of \textsc{Pivoting} are non-probabilistic.% \todo{}

We propose a simple method to solve this problem: we convert scores without probabilistic interpretation to ones that are scaled to the zero-one simplex. Given mention $m_i$ and its top-$n$ candidate entity list $\Ev_{i}$ along with their prior scores $\mathbf{P}_i$, the re-calibrated scores are identified as:
\begin{equation}
    p_{i,j}'=\frac{\exp(\gamma \times p_{i,j})}{\sum_{p\in \mathbf{P}_i}\exp(\gamma \times p)}
\end{equation}
where $\gamma$ is a hyper-parameter that controls the difference between scores after taking exponential.  

After the calibration, it is safe to combine prior scores with an average. 
% \subsection{Candidate Generation}
% For candidate generation, we use the zero-shot \textsc{Pivoting} model described in the previous section~\cite{rijhwani19aaai}.  By using this, we fully remove the dependency on $\mathbbm{M}$ in the candidate generation process. Note that this system does not perform collective inference over the whole document -- it predicts candidates for each mention independently. Our proposed model uses these candidates in a document-level inference approach.

\subsection{Feature Design}\label{feature}
Next, we introduce the feature set for our inference model, which includes features inspired by previous work \cite{sil2016one, ganea2016probabilistic, pan2017cross}, as well as a novel set of features specifically designed to tackle the low-resource scenario. The formulation and resource requirements of unary features are shown in the top half of Table \ref{tab:1} and those of binary features are shown in the bottom half of Table \ref{tab:1}. %The definition of unary and binary features are mentioned in Section \ref{sec:base_inference}. 

% Similar to \citet{pan2017cross}, we use $f_l^1(e_{i,j})$ -- the mention-entity prior probability that indicates how often $e_{i,j}$ is linked when mentioning $m_i$. Additionally, we use $f_g^1(e_{i, j}, e_{k, m})$ -- the co-occurrence probability of entity $e_{i,j}$ and entity $e_{k, m}$.  

% Because of the resource dependency they have, the availability of \textsc{Base} features described in Section \ref{baseline} are affected by the existence of resources. Without access to $\mathbbm{W}_{\textrm{src}}$ and $\mathbbm{M}$, we are unable to obtain $f_l^1$, which~\citet{upadhyay2018joint} argue is an essential indicator of entity-mention coherence.
% In the EL and XEL literature, almost all models, even those that aim to be ``zero-shot'', take advantage of this feature \cite{upadhyay2018joint,sil2018neural};. Without it, the linking capacity of many systems degrades drastically~\cite{upadhyay2018joint}. We argue that, to compensate for the absence of important features under resource constraints, it is necessary to design more intelligent features from the source document $D$ and the only language-invariant resource $\mathbbm{W}_{\textrm{eng}}$. 

We design these features at two levels: (1) At the entity-entity level, even though $f_g^1$ is widely used in different XEL systems, it is noisy and sparse. 
To overcome noise we calculate the smoothed Positive Pointwise Mutual Information (PPMI) \cite{church1990word,ganea2016probabilistic} between two entities as $f_g^2$ (second row of bottom half of Table \ref{tab:1}). Compared to pure co-occurrence probability $f_g^1$, this is a more precise estimation of how much more the two entities co-occur than we expect by chance. To tackle sparsity, we incorporate English entity embeddings of \citet{yamada2017learning} and use the embedding similarity between two entities as another dimension of entity relatedness. This is denoted by $f_g^3$, shown in the third row of the bottom half of Table \ref{tab:1}. (2) At the entity-mention level, we consider the number of mentions an entity is ``related to'' as $f_l^3$ (third row of the top half of Table \ref{tab:1}), where we consider an entity $e_{i,j}$ ``related to'' mention $m_k$ if it co-occurs with any candidate entity of $m_k$. 

We intentionally avoid any feature that takes word in the context into consideration. They are heavily reliant on $\mathbbm{W}_{\textrm{eng}}$ and $\mathbbm{M}$ and thus largely weaken the transferability of the model. 

We name our proposed feature set that includes all features listed in Table \ref{tab:1} as \textsc{Feat}.
% The feature set that removes $f_l^1$ is called \textsc{FeatNP}. Similarly, the feature set without $f_l^1$ in our base model is called \textsc{BaseNP}.  

\subsection{\textsc{Burn}: Feature Combination Model}\label{sec:burn}
With the growing number of features, we posit that a linear model with greedy entity pair selection (Section \ref{sec:base_inference}) is not expressive enough, and may understate the advantage of a rich feature set. \citet{yamada2017learning} use Gradient Boosted Regression Trees (GBRT; \citet{friedman2001greedy}) to combine features. However, incorporating this algorithm would not allow for end-to-end training and thus constraints the flexibility of the model. Instead, \citet{ganea2016probabilistic} and \citet{ganea2017deep} propose using Loopy Belief Propagation (LBP; \citet{murphy1999loopy}) to better estimate the global score (Equation \eqref{eq:base_g}). They also use a multi-layer perceptron with non-linear functions to combine local score and global score (Equation \eqref{burn:final}). However, BP is challenging to implement because of a circular dependencies in the graph. 
%\sr{is it "because of" a circular dependency?}. 
In addition, they do not attempt to combine more fine-grained features (e.g. unary feature $\mathbf{\Phi}(e_{i,j})$) non-linearly.  
% \gn{Need to remind people why previous work was limited to linear models in the first place; be carefully about the claim. check it later}.

In our work, we propose a \emph{belief update recurrent network} (\textsc{Burn}) that combines features in a non-linear and iterative fashion. Compared to existing work \cite{naradowsky2016represent, ganea2016probabilistic, ganea2017deep} as well as our base model, the advantages of \textsc{Burn} are: (1) it is easy to implement with existing neural network toolkits, (2) parameters can be learned end-to-end, (3) it considers non-linear combinations over more fine-grained features and thus has potential to fit more complex combination patterns, (4) it can model (distance) relations between mentions in the document. 
%This method is shown in Figure \ref{fig:1} 
%\sr{can we briefly say all this in the intro? it sounds very cool!}.
%\gn{Make the contrast to the inference methods in previous work. Also might be worth pointing out that from an implementation point of view this is relatively easy: just use a neural network toolkit.}.


% \begin{figure*}[t]
% \centering
% \includegraphics[width=0.7\textwidth]{figures/model.png}
% \caption{The architecture of \textsc{Burn}}
% \label{fig:1}
% \end{figure*}

%\sr{can we reference the figure a bit more through the description? if not, we maybe don't need the figure at all}
Given a unary feature vector $\mathbf{\Phi}(e_{i,j})$ with $d_l$ unary features, \textsc{Burn} does not calculates the local score through the linear combination in Equation \eqref{eq:base_l}, but instead by a neural network with two fully connected layers:
\begin{equation}\small
    s_l(e_{i,j}|D)={\Wv_l^2}^T(\sigma({\Wv_l^1}^T\mathbf{\Phi}(e_{i,j}))) + {\Wv_l^3}^T\mathbf{\Phi}(e_{i,j})
\end{equation}
where $\textbf{W}_l^1 \in \mathbbm{R}^{d_l \times h_l}$, $\textbf{W}_l^2 \in \mathbbm{R}^{h_l \times 1}$ and $\textbf{W}_l^3 \in \mathbbm{R}^{d_l \times 1}$. $\sigma$ is the non-linear function, for which we use leaky rectified linear units (Leaky ReLu; \citet{maas2013rectifier}). We add a linear addition of the input to alleviate the gradient vanishing problem. Equation \eqref{eq:base_e} is revised in a similar way. 

The difficulty of a disambiguation model that considers mention evidence is that there may be a large number of entity candidates for each mention, many of which may be noise.
% While Equation \eqref{eq:base_m} prevents the base model from enumerating all combinations of entities in the document, 
%it greedily looks for the related entity $e_{k, w}$ of mention $m_k$ without considering its correctness. 
% its greedy strategy is sub-optimal. Considering mention evidence from $m_k$ to $e_{i, j}$, if the entity with highest entity pair score ($s_e(e_{i,j}, e_{k,w})$) is in fact not the correct linked entity of $m_k$, the mention evidence becomes noise, instead of a helpful clue for disambiguation.
\textsc{Burn} solves this problem by weighting $s_e(e_{i,j}, e_{k,w})$ with the current entity probability $p(e_{k,w}|D)$.
The evidence from $m_k$ is now defined as:
\begin{equation}\label{eq:mention_semantic_related}
 s_m(m_k, e_{i, j}) = \sum_{w=1}^{|C_k|}s_e(e_{i, j}, e_{k, w})p(e_{k, w}|D)   
\end{equation}
% In this way, even if the correct linked entity $e_k^*$ does not have the highest score with $e_{i,j}$, its influence of could be amplified by its probability $p(e_k^*|D)$, making it dominate $m_k$'s mention evidence. On the other hand, the influence of wrong candidate entities would be shadowed because of their low probabilities.

Instead of simply averaging mention evidence in Equation \eqref{eq:base_g}, we also use a gating function to control the importance of the $m_k$'s mention evidence when disambiguating $m_i$. The gating function $g$ is essentially a lookup table that takes the distance\footnote{We define the distance of two mentions as the number of words in between} between two mentions as the key and returns a scalar. We train this lookup table along with all other parameters of the model. The updated global score is defined as: 
\begin{equation}\label{eq:global_score}
    s_g(e_{i,j}|D)=\sum_{k \neq i}g_m(m_i, m_k)s_m(m_k, e_{i, j})
\end{equation}
The motivation for this gating function is that a mention is more likely to be coherent with a nearby mention than a distant one. 
We assume that this is true for almost all languages, and thus will be knowledge that can be transferred even without training data in the language to be processed. 

As shown in Equation \eqref{eq:mention_semantic_related}, there is a circular dependency between entities. To solve this problem, we iteratively update the probability of entities until convergence or reaching a maximum number of iterations $T$. In iteration $t$, the calculation of $s_m$ will use entity probabilities from iteration $t-1$. The revised Equation \eqref{eq:mention_semantic_related} is as follows:
\begin{equation}
 s_m^{t}(m_k, e_{i, j}) = \sum_{w=1}^{|C_k|}s_e(e_{i, j}, e_{k, w})p^{t-1}(e_{k, w}|D)
\end{equation}
Unrolling this network through iterations, we can see that this is in fact a recurrent neural network, hence the method name.  

The weights of \textsc{Burn} are learned end-to-end with the objective function:
\begin{equation}
    L(\mathcal{D}, \mathcal{E})=-\sum_{D\in \mathcal D}\sum_{m_i \in D}\log(p^{T}({e}_i^*|D)).
\end{equation}

\noindent
\textbf{Training \textsc{Burn}}: 
% As shown in Tables~\ref{tab:1}, we only require English Wikipedia for creating the features, except for the mention-entity prior probability, which is required for the \textsc{Feat} feature set, but not \textsc{FeatNP} feature set. Additionally, in the case of \textsc{FeatNP}, we do not require any annotated EL data or other resources in the source language. 
As discussed above, the disambiguation model is fully language-agnostics and it does not require any annotated EL data or other resources in the source language. The model weights $W_l$, $W_g$ and the the lookup table $g_m$ of gating function are trained on the TAC-KBP 2010 English training set~\cite{ji2010overview} \emph{only} and used as-is or another language. We use TAC-KBP 2012 English test set \cite{mayfield2012overview} as our development set. 













==> 5.relatedwork.tex <==
\section{Related Work}
\label{sec:related}
% \sz{maybe we could temporally delete related work and add it back in the camera-ready version?}
% mainly two parts, 1) the design of our model, local, global scores, inference - show our model intentionally avoid some features and also show the efficiency of our inference model; 2) XEL setting, show how unwarranted assumptions has been made and show how our model better use scarce but existent resource (compare to Pan)

\gn{I'd suggest maybe splitting these up into paragraphs with explicit headers. Maybe saying something like: ``In this section, we overview the related work in XEL from several dimensions corresponding to each component of the XEL system: (1) candidate generation, (2) featurization, and (3) inference for disambiguation, and (4) resource usage.'' This might make things more clear and clean.}

Previous (X)EL works mainly focus on the design of the \emph{disambiguation} model, which could be further decomposed to the design of (unary and binary) features and inference algorithms. A unary feature mainly measures the compatibility between an entity and the context where it lies. This feature often includes the salience of an entity~\cite{bunescu2006using,cucerzan2007large,dredze2010entity,hoffart2011robust, ganea2017deep,yamada2017learning, pan2017cross, sil2018neural} and the similarity between the context and an entity's description~\cite{cheng2007entityrank,ganea2017deep, yamada2017learning, sil2018neural, upadhyay2018joint}. On the other hand, a binary feature quantifies the coherence of entities in the document. Common binary features come from KB statistics~\cite{cucerzan2007large, ganea2016probabilistic, globerson2016collective, pan2017cross} or learnt entity embeddings~\cite{yamada2017learning, ganea2017deep, le-titov-2018-improving}. Our collection of features is largely inspired by these existing works with an intentional ignorance of resource-heavy features like context-description similarity. 

In terms of inference algorithms, while some works~\cite{yamada2017learning, sil2018neural, upadhyay2018joint} entails mentions independently, others attempt to collectively resolve all mentions. These algorithms include random graph walks~\cite{guo2018robust}, pagerank~\cite{pershina2015personalized}, loopy belief propagation~\cite{ganea2016probabilistic, ganea2017deep, le-titov-2018-improving}. Our proposed \textsc{Burn} generally follows the collective inference manner. However, it is easier to implement with existing neural network toolkits and could fix more complex feature combination patterns because of its non-linearity. 

In addition to standard (X)EL, \citet{pan2017cross,sil2018neural, upadhyay2018joint} explore this problem in low- and zero-resource settings. \citet{sil2018neural, upadhyay2018joint} simulate the resource scarce scenario with data in high-resource languages (e.g. Spanish and Chinese). They mainly consider resource constraints during \emph{disambiguation} process with high quality candidate entity lists. However, we show that the resource availability in fact strongly deteriorates the quality of candidate lists, and thus the ideal testbed for the disambiguation model solely in true low-resource settings is not likely. \citet{pan2017cross} bridges the resource gap between the LRL and the HRL by translating LRL mentions to English with the help of bilingual entity maps $\mathbbm{M}$. They then use English EL model~\cite{pan2015unsupervised} to generate candidate entities and perform disambiguation. While this model avoids the use of $\mathbbm{W}_{\textrm{src}}$, in low-resource settings, we empirically observe its sub-optimal candidate generation performance compared to \textsc{WikiMention} with this very small $\mathbbm{W}_{\textrm{src}}$. %\sz{are claims too aggressive?}

% \section{Training Details}\label{train_detail}
% All models are implemented in the PyTorch Framework~\cite{paszke2017automatic}. The size of the pre-trained entity embeddings\footnote{https://wikipedia2vec.github.io/wikipedia2vec/\\pretrained/} is 300, trained with a window size set to 15 and negative sample set to 15.  The hidden state of both unary and binary features are set to 128, the dropout rate is set to 0.5. For the gating function, we set mention distances that are larger than 50 tokens are to 50, then bin the distance with a bin size of 4. We only consider the 30 nearest context mentions for one mention. The maximum number of iterations for inference is set to 20. We use Adam optimizer with the default learning rate (\texttt{1e-3}) to train the model. The $\gamma$ of calibrated candidate combination is set to 1.
% % The model is trained on the TAC-KBP 2010 English training set~\cite{ji2010overview} and hyper-parameters are tuned on the TAC-KBP 2012 English evaluation dataset~\cite{mayfield2012overview}.
% % In the candidate generation process, we set $K=30$ for all languages. The $\gamma$ in Section 4.1 is set to 1.
\section{\textsc{Pivoting} Candidate Generation}

We select training languages for the pivoting model based on language family similarity with the source language in question. The models are tuned on a validation set from Wikipedia, which has no overlap with our DARPA test datasets.
The training languages we choose are -- Amharic (for Tigrinya), Somali (for Oromo), Kirundi (for Kinyarwanda) and Hindi (for Sinhala)~\cite{rijhwani19aaai}. 

We train the models on bilingual entity maps obtained from Wikipedia language links, on the transfer language \emph{only}, to maximize cosine similarity between entity encodings. No data in the source language is used for training.


==> binary_table.tex <==
\begin{table*}[t]
  \centering
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{c|c|c|c}
  \toprule
  \textbf{Symbol} & \textbf{Feature Name} & \textbf{Equation} & \textbf{Resource} \\
  \midrule
  
  \rowcolor{Gray}
  $f_g^1(e_i, e_j)$ & Co-occurrence probability & $\log(\max(\frac{c(e_i, e_j)}{c(e_i)}), \epsilon)$ & $\mathbbm{W}_{\textrm{eng}}$ \\
  
  $f_g^2(e_i, e_j)$ & Positive Pointwise Mutual Information (PPMI) & $\max (\log_2 (\frac{p(e_i, e_j)}{p'(e_i)p'(e_j)}), 0)$ & $\mathbbm{W}_{\textrm{eng}}$  \\
  
  $f_g^3(e_{i}, e_j)$ & Entity embedding similarity & $\text{cosine}(V_{e_i}, V_{e_j})$ & $\mathbbm{W}_{\textrm{eng}}$ \\
  
  $f_g^4(e_i, e_j)$ & Hyperlink count & $\log(\max(\frac{\sum_{e_k \in H_{e_{j}}}\mathbbm{1}(e_i=e_k)}{|H_{e_{j}}|}, \epsilon)$ & $\mathbbm{W}_{\textrm{eng}}$ \\
  \bottomrule
  
  \end{tabular}%
  }
  \caption{Binary Features. Gray row shows \textsc{Base} feature. $\epsilon$ is set to \texttt{1e-7}; function $c(e_{i}, e_{j})$ returns the count of these two entities co-occurs in any English Wikipedia ($\mathbbm{W}_{\textrm{eng}}$) page; function $p(e_{i}, e_{j})$ is the probability normalized over all entity pairs and $p(e_{i})$ is the probability normalized over all entities with smooth parameter $\gamma=0.75$; $\Vv_{e}$ represents the entity embedding of $e_{i}$; $\Hv_{e_{i}}$ represents a set of entities in $e_{i}$'s English Wikipedia page.} 
  \label{tab:2}
\end{table*}

==> old/7.v0_method.tex <==
\section{Proposed Method}
\gn{``Proposed Method'' is a rather boring section title. Can we make it more interesting?}

\gn{One way to write the paper might be to have Section 2 problem formulation, Section 3 give an example of a baseline resource-rich model (similar to the previous work by Pan et al. or probabilistic bag of hyperlinks), and Section 4 give our proposed model, at each step contrasting to the baseline model and demonstrating how resource requirements are different.}


\subsection{Baseline Model}
Change \eqref{eq:mention_semantic_related} to 
$$s_m(m_k, e_{i, j}) = \max(s_e(e_{i, j}, e_{k, w}))$$

and change \eqref{eq:global_score} to 

$$ s_g(e_{i,j})=\frac{1}{|m|}\sum_{k \neq i}s_m(m_k, e_{i, j}) $$

That is to say, the evidence from another mention is not the Expectation anymore, and all mentions are treated equally. As it does not have circular dependency, there is no need to inference iteratively. This is similar to Section 4.5   Coreference part of \citet{ling2015design}

\sz{I will change the proposed model part as you suggested}

\subsection{Collective Model}
Our goal is to define the conditional probability of each entity given the document $D$. This probability is the softmax probability over all candidate entities from the same mention:
$$p(e_{i, j}|D) =\textrm{softmax}_{m_i}(\textrm{s}(e_{i, j}|D))$$
where $s(e_{i, j}|D)$ is the score for $j$-th candidate entity of $i$-th mention in the document $D$. 

The score $s(e_{i,j}|D)$ for candidate entity $e_{i, j}$ can be decomposed to two parts: local score $s_l(e_{i,j}|D)$ and global score $s_g(e_{i,j}|D)$. They are defined on the log scale and we have
$$s(e_{i, j}|D)=s_g(e_{i, j}|D) + s_l(e_{i, j}|D)$$

\textbf{Local score} $s(e_{i,j}|D)$ of entity $e_{i,j}$ is defined by a unary features vector $\mathbf{\Phi}(e_{i,j}) \in \mathbbm{R}^{d_l}$. Each feature vector contains $d$ unary features and each of them is a numerical value. We will introduce these features in Section 2.3. As the importance of features varies, previous works often assign a weight to each of them. These weights can be set manually or learnt by machine learning method. In our work, we rely on neural network with two fully connected layers to learn the combination of features. With non-linear function, the result combination is often more expressive. What's more, it allows we to train the model end-to-end. 

To be specific, given a unary feature vector $\mathbf{\Phi}(e_{i,j})$, the local score of this entity is defined as:

$$s_l(e_{i,j}|D)={\Wv_l^2}^T(\sigma({\Wv_l^1}^T\mathbf{\Phi}(e_{i,j}))) + {\Wv_l^3}^T\mathbf{\Phi}(e_{i,j})$$

where $\textbf{W}_l^1 \in \mathbbm{R}^{d_l \times h_l}$, $\textbf{W}_l^2 \in \mathbbm{R}^{h_l \times 1}$ and $\textbf{W}_l^3 \in \mathbbm{R}^{d_l \times 1}$. $\sigma_1$ is the non-linear function. In our paper, it refers to leaky rectified linear unit (Leaky ReLu) that is formulated as:

\begin{align*}
\sigma_1(x) = \begin{cases} x  &  \mbox{if} \ \ \mathbf{x}>0 \\ 
0.01x & \mbox{otherwise}
\end{cases}
\end{align*}

We add a linear combination to alleviate the gradient vanish problem. 

\textbf{Global score} $s_g(e_{i, j}|D)$ of entity $e_{i,j}$ measure its comparability with other mentions in the same document $D$. It is the weighted combination of semantic related score $s_m(m_k, e_{i, j})$ between entity $e_{i,j}$ and mention $m_k$ ($m_k \neq m_i$):
\begin{equation}\label{eq:global_score}
    s_g(e_{i,j})=\sum_{k \neq i}g_m(m_i, m_k)s_m(m_k, e_{i, j})
\end{equation}

Here $g_m(m_i, m_j)$ is the gating function that control to importance of mention $m_k$ to disambiguate $m_i$.The function is measured by the distance (in token) between two mentions. We bin our distance into buckets with bin size $b$ and use a lookup table to find its gating value. These values are also learnt end-to-end. The idea behind this gating function is that even a document is often related to on topic, mentions are not necessarily always related to that topic. However, it is still the case that a mention is more likely to be coherent to another mention that is closed to it than mentions that are far away, which is true for almost all languages. 

The semantic related score $s_m(m_k, e_{i, j})$ is calculated as the weighted sum of semantic related score $s_e(e_{i, j}, e_{k, w})$ between $e_{i, j}$ and $e_{k, w}$: 

\begin{equation}\label{eq:mention_semantic_related}
 s_m(m_k, e_{i, j}) = \sum_{w=1}^{|C_k|}s_e(e_{i, j}, e_{k, w})p(e_{k, w}|D)   
\end{equation}

Similar to the calculation of local score, $s_e(e_{i, j}, e_{k, w})$ is produced by a two-layer fully connect Neural network whose input is a binary feature vector $\mathbf{\Psi}(e_{i, j}, e_{k, w})\in \mathbbm{R}^{d_e}$:

\begin{align*}
  s_e(e_{i,j}, e_{k, w})={\Wv_e^2}^T(\sigma({\Wv_e^1}^T\mathbf{\Psi}(e_{i,j}, e_{k, w}))) \\
  + {\Wv_e^3}^T\mathbf{\Psi}(e_{i,j}, e_{k, w})
\end{align*}

where $\textbf{W}_e^1 \in \mathbbm{R}^{d_e \times h_e}$, $\textbf{W}_e^2 \in \mathbbm{R}^{h_e \times 1}$ and $\textbf{W}_e^3 \in \mathbbm{R}^{d_e \times 1}$. $\sigma_1$ is the Leaky ReLu function. We also add the linear combination to alleviate gradient vanish problem. We will discuss the design of $\mathbf{\Psi}(e_{i,j}, e_{k, w})$ in section 2.3.

As equation [] requires the conditional probability of other entities, there is a circle in the dependency (??). To solve this problem, we update this conditional probability iteratively until converge or reach the  maximum iteration. In iteration $i$, we calculate equation [] by using conditional probability from iteration $i-1$:

$$s_m^i(m_k, e_{i, j}) = \sum_{w=1}^{|C_k|}s_e(e_{i, j}, e_{k, w})p^{i-1}(e_{k, w}|D)$$

The goal of the learnt model is to assign maximum probability to gold entity $e_i^*$ of mention $m_i$, thus, the objective function of our model is to minimized the negative log probability of gold entity:

$$L=-\sum_{D\in \mathcal D}\sum_{m_i \in D}\log p(e^*_i|D)$$

\subsection{Feature Description}

In this section, we will describe elements in unary feature vector $\mathbf{\Phi}(e_{i, j})$ and binary feature vector $\mathbf{\Psi}(e_{i, j}, e_{k, w})$. We also list the resources that are required to get the feature. 

The formulation of unary features are showed in Table 1 and the formulation of binary features are shown in Table 2. 

We further explain some features as their equation are not straightforward.
\begin{itemize}
    \itemsep0em 
    \item Relate mention number
    \item Entity embedding similarity
    \item Hyperlink count
\end{itemize}


\input{unary_table.tex}
\input{binary_table.tex}

\subsection{Pivoting Zero-shot Candidate Generation}

In previous works, the candidate generation processed is often treated as a look up process, where given a mention, a list of candidate entities are returned by a dictionary. To build such a dictionary for cross-lingual setting, we should first build a monolingual dictionary from the source language Wikipedia \cite{shen2015entity}, and use corresponding inter-language links to map entities to their English Wikipedia entries \cite{upadhyay2018joint}. However, this process is non-trivial for languages with only few or none pages. Thus, we apply zero-shot pivoting model that is proposed by \citet{rijhwani19aaai} to generate candidate entities for each mention. \todo{introduce pivoting}

\subsection{Heuristic Coreference Resolution}
\todo{Where to put it}


==> old/8.v1_method.tex <==
\section{Baseline Model}
In this section, we introduce examples of previous methods that require the accessibility to $\mathbbm{RC}_1$, $\mathbbm{RC}_2$, $\mathbbm{RC}_3$.
% We gradually make more strict resource availability constraints and incorporate resource-lighted components until reach the minimal resource requirement we are aware of in previous work: ($\mathbbm{RC}_1$, $\mathbbm{RC}_3$).
We use this to devise a baseline model and demonstrate that it is an approximation to existing work \sr{cite?}.
% We further improve the baseline model to accommodate extremely limited resource setting. The details of our proposed methods are introduced in Section \ref{model}.  

\subsection{Candidate Generation}\label{sec:wikimentin}
\textsc{WikiMention}: With full access to resources we list above, there is a straightforward approach to the candidate generation process for XEL. A monolingual mention-entity map can be extracted from $\mathbbm{RC}_2$ by finding all article links in Wikipedia, and using the anchor text as $m$ and the linked article as $e^s$. These entities are then redirected to English Wikipedia with $\mathbbm{RC}_3$ to obtain $e$. For instance, because mention ``丹麦'' is linked to 丹麦人\footnote{https://zh.wikipedia.org/wiki/丹麦人}  in one Chinese Wikipedia page, Danes\footnote{https://en.wikipedia.org/wiki/Danes} is one candidate entity of ``丹麦'' \sr{can we make a figure of this?}. We use the existing implementation by~\citet{upadhyay2018joint}.\footnote{https://github.com/shyamupa/wiki\_candgen}
% To expand coverage, for a mention $m_i$ in the document, we also consider the candidate entities of any other mention $m_k$ if $m_i$ is the substring of $m_k$. \gn{Connecting this to the example above would be helpful}. 

\texttt{WikiMention} works to some extent, but is heavily reliant on having a large entity map, namely source-language Wikipedia $\mathbbm{RC}_2$ and Bilingual entity map $\mathbbm{RC}_3$, which we found constraining even in high-resource languages. To work in more realistic resource-limited settings, \citet{pan2017cross} propose a translation-based method that can get rid of the necessity for $\mathbbm{RC}_2$.
In this method, mention $m$ in the source language is first translated to English with the help of bilingual entity map $\mathbbm{RC}_3$.
A list of candidate entities can then be retrieved by referring to the English mention-entity map that is extracted from $\mathbbm{RC}_1$. One side product of this candidate generation method is that we could obtain $f_l^1$ without accessing $\mathbbm{RC}_2$ too. This is called \texttt{Translation} in the paper. To our best knowledge, this is the method with the lowest resource dependency that performs full entity linking and disambiguation that we could find in the literature \gn{We need to make sure that it's clear why we don't consider Shruti's method to be ``prior work''}. 

\subsection{Inference}\label{sec:base_inference}
Similarly to previous work, the score of associating a mention with an entity is measured by two components: \emph{local score} that indicates the similarity between an entity and the local context it lies; \emph{global score} that quantifies the similarity between an entity and other linked entities in the same document. On the log scale, the score of each entity is defined as:
\begin{equation}\label{burn:final}
    s(e_{i, j}|D)=s_g(e_{i, j}|D) + s_l(e_{i, j}|D)
\end{equation}

The local score is the linear combination of a list of unary features $f_l^i(e_{i,j}) \in \mathbf{\Phi}(e_{i,j})$, where a unary feature function takes one argument $e_{i,j}$ and returns a value that only related to this entity (\citet{pan2017cross}; \citet{globerson2016collective} ):
\begin{equation}\label{eq:base_l}
    s_l(e_{i,j}|D)={\Wv_l^T}\mathbf{\Phi}(e_{i,j})
\end{equation}
Where $\textbf{W}_l \in \mathbbm{R}^{d_l \times 1}$ and $d_l$ is the number of unary features in the vector. 

On the other hand, the calculation of global score is not as straightforward as local score. At first place, we measure the entity pair score between two entities by the linear combination of a list of binary features $f_g^i(e_{i,j}, e_{k, w}) \in \mathbf{\Psi}(e_{i, j}, e_{k, w})$. Each binary feature function $f_g^i(e_{i,j}, e_{k, w})$ takes two arguments and returns a value that indicating the relatedness between two entities, we denote the entity pair score by $s_e(e_{i,j},e_{k, w})$:
\begin{equation}\label{eq:base_e}
    s_e(e_{i,j}, e_{k, w})={\Wv_g^T}\mathbf{\Psi}(e_{i,j}, e_{k, w})
\end{equation}
Where $\textbf{W}_g \in \mathbbm{R}^{d_g \times 1}$ and $d_g$ is the number of binary features in the vector. 

This score is still not ready to be the final global score for $e_{i,j}$, and it should be further represented as the mention evidence that suggests the relatedness between an entity and a mention. The mention evidence is denoted by $s_m(m_k, e_{i,j})$. Similar to \citet{ling2015design} and \citet{globerson2016collective}, we greedily look for entity pairs with highest entity pair score and ignore remaining ones:
\begin{equation}\label{eq:base_m}
    s_m(m_k, e_{i,j}) = \max_{e_{k,w}\in \Ev_{k}}(s_e(e_{i, j}, e_{k, w}))
\end{equation}
The global score is then defined as the average of mention evidence of the document:
\begin{equation}\label{eq:base_g}
    s_g(e_{i,j}|D)=\frac{1}{|\Mv_{D}|}\sum_{k \neq i}s_m(m_k, e_{i,j})
\end{equation}
The more sophisticated way to calculate global scores is  in Section \ref{sec:burn}

Similar to \citet{pan2017cross}, there are mainly two features in our base model: $f_l^1(e_{i,j})$: the mention-entity prior probability, and $f_g^1(e_{i, j}, e_{k, m})$: the co-occurrence probability of entity $e_{i,j}$ and entity $e_{k, m}$ of mention $m_k$. We show detailed formulations of these features in Table \ref{tab:1} and Table \ref{tab:2}. For simplicity, we omit arguments of each feature function in the following paragraphs. 


\input{unary_table.tex}
\input{binary_table.tex}

\section{Collective Minimal Resource Model}\label{model}
As shown in the previous section, the minimal resource requirement of existing XEL systems are English Wikipedia ($\mathbbm{RC}_1$) and bilingual entity map ($\mathbbm{RC}_3$). However, even the availability of $\mathbbm{RC}_3$ is scarce for most living languages, making it almost impossible to directly apply these systems to languages with extremely limited resources. In addition, even in languages where source Wikipedia ($\mathbbm{RC}_2$) is available, often it can be small to the extent where it is not possible to rely on this resource heavily for either candidate generation or feature extraction.

In this section, we introduce an XEL system that requires only the language-invariant resource $\mathbbm{RC}_1$, a first step towards real zero-resource XEL. 

\subsection{Candidate Generation}
For candidate generation zero-shot entity linking model proposed by \citet{rijhwani19aaai}. \gn{Here it is important to be clear that this does not perform inference, only calculates the independent prior probability.}
\todo{describe the model}. In this way, we could fully remove the dependency on $\mathbbm{RC}_3$ in candidate generation process.

\subsection{Feature Design}
The availability of features is also affected by the existence of resources.
Without the access to $\mathbbm{RC}_2$ and $\mathbbm{RC}_3$, we are not able to obtain $f_l^1$, which has been proved to be a reliable indicator of entity-mention coherence, and achieves non-trivial performance on many benchmark datasets \cite{upadhyay2018joint}.
In the EL and XEL literature, almost all models, even those that aim to be ``zero-shot'' entity linking models, take the advantage of this feature, and without it, the linking capacity of many systems degrades drastically.  

We argue that to compensate for the absence of important feature under resource constraints, it is necessary to mine more intelligent features from the source document $D$ and the only language-invariant resource $\mathbbm{RC}_1$. In our method, we design this set of features at two levels. The details of these features are shown in Table \ref{tab:1} and Table \ref{tab:2}. At the entity-entity level, even though $f_g^1$ is widely used in different XEL systems, it is in fact noisy and sparse. \gn{I think the following explanation would be better if it was done in bullet points, which would help make things more organized:}
To overcome the first problem, we calculate the Positive Pointwise Mutual Information (PPMI) \cite{church1990word} between two entities as $f_g^2$. Compared to $f_g^1$, it is a more precise estimation of how much more the two entities co-occur than we expect by chance. In terms of the second issue, we incorporate entity embeddings proposed by \citet{yamada2017learning} and employ the embedding similarity between two entities as another dimension of entity relatedness. At entity-mention level, we consider the number of mentions an entity related to as $f_l^3$, an entity $e_{i,j}$ is said to relate to mention $m_k$ if it co-occurs with any candidate entity of $m_k$. Our proposed feature set including these features is referred to as \textbf{$\textrm{Feature}^+$}. 


\subsection{Feature Combination}\label{sec:burn}

With the growing number of features, a linear model with greedy entity pair selection is not expressive enough, and may discount the advantage a rich feature set. \citet{yamada2017learning} uses Gradient Boosted Regression Trees (GBRT)\cite{} to combine features. However, incorporating this algorithm would break the end-to-end system and thus constraints the flexibility of the model. Besides, \citet{ganea2017deep} propose to use Belief Propagation (BP; \cite{}) to better estimate the global score (Equation \ref{eq:global_score}). They also considers a multi-layer perceptron with non-linear functions to combine local score and global score (Equation \ref{burn:final}). However, BP is hard to implemented with circular dependency in the graph. In addition, they do not attempt to combine more fine-grained features (e.g. $\Phi(e_{i,j})$) non-linearly.  
\gn{Need to remind people why previous work was limited to linear models in the first place; be carefully about the claim. check it later}.

In our work, we propose a \emph{belief update recurrent network} (\texttt{BURN}) that combines features in a non-linear and iterative fashion. Compared to both existing works and our base model, the advantages of this model are: (1) It is easy to implemented with a neural network toolkit; (2): Parameters could be learnt end-to-end; (3): It considers the non-linear combination over more fine-grained features and thus could probably fit more complex combination patterns; (4): It tries to model more complex relations between mentions in the document. This method is shown in Figure \ref{fig:1}.
%\gn{Make the contrast to the inference methods in previous work. Also might be worth pointing out that from an implementation point of view this is relatively easy: just use a neural network toolkit.}.


\begin{figure*}[t]
\centering
\includegraphics[width=0.7\textwidth]{figures/model.png}
\caption{The architecture of \texttt{BURN}}
\label{fig:1}
\end{figure*}

Instead of a linear combination in Equation \ref{eq:base_l}, given a unary feature vector $\mathbf{\Phi}(e_{i,j})$ with $d_l$ unary features, the local score of this entity is given by a neural network with two fully connected layers:
\begin{equation}\small
    s_l(e_{i,j}|D)={\Wv_l^2}^T(\sigma({\Wv_l^1}^T\mathbf{\Phi}(e_{i,j}))) + {\Wv_l^3}^T\mathbf{\Phi}(e_{i,j})
\end{equation}
where $\textbf{W}_l^1 \in \mathbbm{R}^{d_l \times h_l}$, $\textbf{W}_l^2 \in \mathbbm{R}^{h_l \times 1}$ and $\textbf{W}_l^3 \in \mathbbm{R}^{d_l \times 1}$. $\sigma_1$ is the non-linear function. In our paper, it refers to leaky rectified linear unit (Leaky ReLu). We add a linear combination to alleviate the gradient vanish problem. Equation \ref{eq:base_e} is revised in a similar way. 



While Equation \eqref{eq:base_m} avoid the base model from enumerating all combinations of entities in the document, it greedily looks for the related entity $e_{k, w}$ of mention $m_k$ without considering its correctness. Considering mention evidence from $m_k$ to $e_{i, j}$, if the most related entity is in fact not the linked entity of $m_k$, this mention evidence becomes the noise, instead of a helpful clue for disambiguation. Our \texttt{BURN} solves this problem by weighting $s_e(e_{i,j}, e_{k,w})$ with $p(e_{k,w}|D)$. The evidence from $m_k$ is now defined as:
\begin{equation}\label{eq:mention_semantic_related}
 s_m(m_k, e_{i, j}) = \sum_{w=1}^{|C_k|}s_e(e_{i, j}, e_{k, w})p(e_{k, w}|D)   
\end{equation}
In this way, even the correct linked entity $e_k^*$ does not have the highest score with $e_{i,j}$, the influence of this score could be amplify by its probability $p(e_k^*|D)$, making it dominate $k_k$'s mention evidence. 

Instead of averaging mention evidence in Equation \ref{eq:base_g}, we also use a gating function to controls the importance of the $m_k$'s mention evidence to disambiguate $m_i$. The gating function takes the distance between two mentions as argument. The updated global score is defined as: 
\begin{equation}\label{eq:global_score}
    s_g(e_{i,j})=\sum_{k \neq i}g_m(m_i, m_k)s_m(m_k, e_{i, j})
\end{equation}
The idea behind this gating function is that even a document often talks about one topic, mentions are not necessarily always related to that topic. A mention is more likely to be coherent to a nearby mention than a distant one. This is true for almost all languages. 

As shown in Equation \ref{eq:mention_semantic_related}, there is a circular dependency between entities. To solve this problem, we iterativly update the probability of entities until converge or reach maximum iteration. That is to say, in iteration $t$, the calculation of $s_m$ will use entity probabilities from iteration $t-1$. The revised Equation \ref{eq:mention_semantic_related} is as following:
\begin{equation}
 s_m^{t}(m_k, e_{i, j}) = \sum_{w=1}^{|C_k|}s_e(e_{i, j}, e_{k, w})p^{t-1}(e_{k, w}|D)
\end{equation}
Unrolling this network through iteration, it is in fact a recurrent neural network.  

The weights of \texttt{BURN} are learnt end-to-end with an objective function:
\begin{equation}
    L=-\sum_{D\in \mathcal D}\sum_{m_i \in D}\log(p({e}_i^*))
\end{equation}














==> result_eng.tex <==
\begin{table}
  \centering
  \begin{tabular}{ccccc}
  \toprule
  \textbf{System} & zh & es & en\\
  \midrule
%   \citet{yamada2017learning} & 85.2 \\
%   \citet{globerson2016collective} & 87.2 \\
%   \citet{sil2018neural} & 87.4 \\
%   $\textrm{Feature}^+$ + \texttt{BURN} & 87.0 \\
%   \midrule
%   \midrule
  SOTA & 86.0 & \textbf{84.4} & \textbf{84.3}  \\
  \textsc{Base} + \textsc{Greedy} & 85.5 & 80.6 & 77.5\\
  \textsc{Feat} + \textsc{Greedy} & 86.7 & 81.1 & 79.8\\
  \textsc{Base} + \textsc{BURN} & 86.8 & 80.5 & 79.7\\
  \textsc{Feat} + \textsc{BURN} & \textbf{87.1} & 81.4 & 83.8 \\
  \bottomrule
  \end{tabular}
  \caption{Accuracy (\%) of Chinese and Spanish; \emph{In-KB} accuracy of English. The SOTA model refers to \citet{upadhyay2018joint} for Chinese and Spanish; It refers to \citet{globerson2016collective} for English.}
  \label{tab:high_resource}
\end{table}

==> result_with_shyam.tex <==
\begin{table}[tb]
  \centering
  \resizebox{\columnwidth}{!}{%
  \begin{tabular}{p{0.5cm}p{0.4cm}p{0.5cm}cccc}
  \toprule
 $\mathbbm{W}_{\textrm{src}}$ & $\mathbbm{M}$ &  $\mathbbm{E}$ & System & es & zh \\
  \midrule
  \checkmark & \checkmark & \checkmark & \textsc{Xelms} & 84.4 & 86.0 \\
   &   & \checkmark & \textsc{Xelms}-\textbf{RL} & $\textrm{53.5}$ & $\textrm{55.9}$ \\
  \midrule
  \checkmark & \checkmark &            & \textsc{Feat} + \textsc{Burn} & 81.4 & 87.1 \\
  & & & \textsc{Feat\textbf{NP}} + \textsc{Burn} & $\textrm{75.9}$ & $\textrm{84.1}$ \\
  \bottomrule
  \end{tabular}%
  }
  \caption{Accuracy (\%) on TAC-MUL. \textsc{Xelms}-\textbf{RL} refers to Resource-Limited version of \textsc{Xelms}. All systems shown use $\mathbbm{W}_{\textrm{eng}}$. The last row represents our proposed model using no additional resources.}
  \label{tab:4}
\end{table}

==> wiki_size.tex <==
\begin{table}[tb]
  \centering
  \begin{tabular}{l | c c c c}
  \toprule
  \textbf{Language} & ti & om & rw & si\\
  \midrule
  \textbf{Wikipedia Size} & 168 & 775 & 1822 & 15050 \\
  \bottomrule
  \end{tabular}
  \caption{Num. of articles in each language's Wikipedia
  }
  \label{tab:wiki_size}
\end{table}
